When to Give Up on a Parallel Implementation

In the Serial Parallel Decision Problem (SPDP), introduced by Kuszmaul and Westover [SPAA'24], an algorithm receives a series of tasks online, and must choose for each between a serial implementation and a parallelizable (but less efficient) implementation. Kuszmaul and Westover describe three decision models: (1) \defn{Instantly-committing} schedulers must decide on arrival, irrevocably, which implementation of the task to run. (2) \defn{Eventually-committing} schedulers can delay their decision beyond a task's arrival time, but cannot revoke their decision once made. (3) \defn{Never-committing} schedulers are always free to abandon their progress on the task and start over using a different implementation. Kuszmaul and Westover gave a simple instantly-committing scheduler whose total completion time is $3$-competitive with the offline optimal schedule. They conjectured that the three decision models should admit different competitive ratios, but left upper bounds below $3$ in any model as an open problem. In this paper, we show that the powers of instantly, eventually, and never committing schedulers are distinct, at least in the ``massively parallel regime''. The massively parallel regime of the SPDP is the special case where the number of available processors is asymptotically larger than the number of tasks to process, meaning that the \emph{work} associated with running a task in serial is negligible compared to its \emph{runtime}. In this regime, we show (1) The optimal competitive ratio for instantly-committing schedulers is $2$, (2) The optimal competitive ratio for eventually-committing schedulers lies in $[1.618, 1.678]$, (3) The optimal competitive ratio for never-committing schedulers lies in $[1.366, 1.500]$.

==> other/doa_pwo_awake.tex <==
\section{ $O(\sqrt{p})$ competitive decide on arrival, parallel work oblivious scheduler }

First we consider completion time. Then we show that this algorithm can easily be adapted  to work for awake time as well.

Algorithm:
We will consider tasks to be the same size if they have serial work differing by a factor of $2$; rounding the sizes of our tasks up by $2$x can't hurt our awake time by more than $2$x.
For the first $\sqrt{p}$ tasks of each type that we see we run them in parallel. 
All remaining tasks of this type are run in serial.

Analysis:
Let $\sigma_k$ be the largest serial task that OPT runs. 
Let $\sigma_j$ be the largest serial task that we run.
Let $f_*$ be the time when the final task arrives.
Let $m_i$ be the number of tasks of type $\sigma_i$.
We can bound our completion time by:

$$T_{US}\le f_* + \max(\sigma_j, \sum_{i\le k} \left( \pi_i/\sqrt{p}  + m_i \sigma_i/p\right) + \sum_{i>k} m_i \pi_i/p  ).$$

The huge sum is clearly an upper bound on the work that we perform, and we are either bottle-necked by a single task or by work. 

Now we give lower bounds on OPT's work:
We are considering completion time:
$$T_{\opt} \ge f_*.$$
OPT runs all tasks of type $i>k$ in parallel:
$$T_{\opt}\ge \sum_{i>k} m_i \pi_i/p.$$
The fact that we ran $\sigma_j$ in serial means that there were at least $\sqrt{p}$  tasks of commensurate type:
$$T_{\opt} \ge \sigma_j/\sqrt{p}.$$
Of course
$$T_{\opt}\ge \sum m_i \sigma_i/p.$$
Finally, 
$$\sum_{i\le k} \pi_i/\sqrt{p} \le \sqrt{p}\sum_{i\le k} \sigma_i \le (2\sqrt{p}) \sigma_k \le (2\sqrt{p})T_{OPT}.$$
Combining the observations we see that 
$$T_{US}\le O(\sqrt{p} T_{\opt})$$

\paragraph{handling awake time}
The above analysis was for handling completion time.
Now we show how to handle awake time. 

WLOG we assume that the input TAP doesn't result in US having any gaps. 
However, on the input TAP OPT may have gaps. 

Our solution is as follows:
Whenever we detect that OPT has finished all present tasks we put our currently running tasks "in the background". In particular this means that when more tasks more we don't remember anything about how we handled the previous tasks. And, the background tasks only run on idle processors, and the way they run is by sharing the idle processors as best they can.
With this strategy it is fairly clear that we aren't so sad about the gaps.

Thus we have
\begin{proposition}
    There is an $O(\sqrt{p})$ competitive scheduler for PWO plus DoA
\end{proposition}

\begin{proposition}
    There is no $o(\sqrt{p})$ competitive scheduler for PWO plus DoA.
\end{proposition}
\begin{proof}
    $\sqrt{p}$ tasks arrive at the beginning, all with serial work $1$.
Then, it could be the case that they are perfectly scalable, in which case you would lose by a factor of $\sqrt{p}$ if you choose to serialize any of them.

On the other hand, they could be perfectly not scalable, in which case you would lose by a factor of $\sqrt{p}$ if you parallelize all of them.

You can't win them all!
\end{proof}


==> other/dtaps.tex <==
\section{DTAPs}
\todo{Define DTAPs}
\todo{Say that KW had tight analysis in the offline case (although only on arxiv).}
\todo{Say that they left it as an open q to analyze offline case.}

\subsection{Exactly Solving Offline DTAPs is Strongly NP-Hard}

\begin{fact}
Exact 3 cover (X3C) is a classic NP-hard problem. 
The problem is, given a 3-regular hypergraph, find a set of half of the hyperedges that hits every vertex exactly once. Or maybe I'm not quite remembering correctly. 
\end{fact}

\begin{theorem}
Exactly computing the optimal awake time for a DTAP is strongly NP-hard, even in the width-zero, arrival time zero setting and when we restrict to DTAPs where all connected components are chains. 
\end{theorem}

\begin{proof}
Let $G= (U, E)$ be our X3C instance, and let $m = |E|, n = |U|$. Identify $U$ with $[n]$.
For each hyperedge in our hypergraph, we create a chain. At the start of the chain is a task with parallel work $1$ and serial work $m/2-XXX$. 

Then, we put ``kebobs'' after the first task. A kebob for hyper edge $(i,j,k)$ with $i<j<k$ is the following chain of tasks: 
\begin{itemize}
\item $i$ forced serial time, 
\item $1$ forced parallel time
\item $j-i-1$ forced serial time
\item $1$ forced parallel time
\item $k-j-1$ forced serial time.
\end{itemize}

\textbf{TODO:} need to change the scale... the kebobs are supposed to be tiny compared to the rest of the stuff

The claim is that if you choose to serialize  $1/2$ of the chains corresponding to an X3C solution, then you will be able to finish the TAP in time XXX, and otherwise you will not. 

To check the ``otherwise you will not'' clause we consider the possible things that the scheduler could do.  
\begin{enumerate}
\item The scheduler could decide to serialize the first task in more than $m/2$ of the chains. This would instantly destroy them. 
\item The scheduler could decide to serialize the first task in less then $m/2$ of the chains, or choose to serialize the first task in $m/2$ of the chains in such a way as to not correspond to an X3C solution. Then, we will get behind in one of the kebobs because we will have multiple units of parallel work at the same time. There is no way to recover from getting behind in a kebob.
\end{enumerate}
\end{proof}

\textbf{Remark:} This probably also works for the non-width zero setting. 
Setting $p$ to be really huge probably does it. Maybe can even get away with $p=2$.

\subsection{Approximation Schemes for Simple DTAPs}

\begin{theorem}
Suppose you have a DTAP where all connected components have size at most some constant $L$. Then, for any constant $\eps>0$, there is a polynomial time $1+\eps$ approximation algorithm for optimizing awake time.  
\end{theorem}

\begin{proof}
First, we round the parallel sizes to be multiples of $T\eps/n$; this increases the completion time by at most $T\eps$. 
Suppose we are trying to decide whether the DTAP can be performed in time $T(1+\eps)$ assuming it can be completed in time $T$. If there is a schedule requiring time $T$, then there is a schedule requiring time at most $T(1+2L\eps)$ where all serial tasks start at times which are integer multiples of $\eps T$, even if we round the serial task sizes up to be multiples of $\eps T$. We now show how to find some such schedule given that one exists.

By scaling we assume $T=1$.
Let $N = \lceil \eps^{-1}\rceil +2L$.
The ``relevant times'' (i.e., times when serial tasks can start) are $\eps\cdot [N]\cup 0$.

Define a \textbf{task completion strategy} as follows:
\begin{itemize}
\item Assign each task an interval in which it promises to finish. This interval is a sub-interval of $[0,N]$ where both endpoints are integral.
\item The assigned intervals must have the property that each task's interval starts after all the tasks that it depends on have promised to finish.
\end{itemize}

We say that a task completion strategy is \textbf{good} if it is possible to complete all tasks during their promised completion intervals.

\textbf{Claim 0:} We can efficiently check if a task completion strategy is good. 
\textbf{Proof:} Given a task completion strategy it is pretty clear how you should run the tasks: prioritize things that have promised to finish earlier. If this simple greedy strategy fails then it is impossible for the task completion strategy to be good. 

\textbf{Claim 1:} The existence of a schedule where serial tasks start at relevant times that achieves completion time $N$ implies the existence of a good task completion strategy. 
\textbf{Proof:} 
Make the promised completion interval of each task be the smallest integer-endpoint interval in which it completes. This is clearly a good task completion strategy.

\textbf{Claim 2:} The existence of a good task completion strategy implies the existence of a schedule with completion time at most $N$.
\textbf{Proof:}
By definition of a good task completion strategy we can run the tasks so that they all complete within their promised completion intervals, which in particular all end before $N$.

\textbf{Claim 3:} We can efficiently determine whether there is any good task completion strategy. 
\textbf{Proof:} 
Here's a pretty silly way to do it:
DP[current chain index, amount of work promised in each of the $\binom{N}{2}$ possible intervals]
To update for a new chain:
\begin{enumerate}
\item Iterate over all $2^L$ possibilities for which tasks in the chain to serialize and which ones to parallelize.
\item Iterate over all $\binom{N}{2L}$ ways to choose promise intervals for the tasks in the chain. 
\item For any such combinations which are reasonable (serial works fit in the intervals), add the promised parallel works to the appropriate intervals.
\end{enumerate}

Combining all the claims, we see that to check whether the DTAP can be completed in time $N$ we can check for the existence of a good task completion strategy, which can be done efficiently. 
\end{proof}

\begin{theorem}
Suppose the DTAP is a union of $k$ chains. 
Fix constant $\eps>0$. There is a $1+\eps$ approximation for the awake time of this DTAP with running time $n^{O_{\eps,k}(1)}$.
\end{theorem}

\begin{proof}
Suppose we are trying to decide whether the DTAP can be performed in time $T(1+\eps)$ assuming it can be completed in time $T$. By rescaling we may assume $T=1$. 
If the DTAP can be completed in time $1$, then there is a schedule with completion time at most $1+2\eps$ where all tasks start at times which are multiples of $\eps/n$ even if we round up the works of all tasks to be multiples of $\eps/n$. 

Now we do a DP. The index for our DP is the current time, our progress into each chain, and our progress into the task currently live from the chain. This gives running time $(n/\eps)^{O(k)}$.
\end{proof}

% \section{Next up}
% We were trying the following problem:

% \begin{theorem}
% Can you do a $2+\eps$-approximation for chains?
% \end{theorem}

% \begin{proof}[Attempt]
% Let $1$ be the goal end time. 
% \textbf{Observation:} WLOG can assume no tasks of size $<\eps/n$
% We can geometrically discretize. This isn't super great yet. 
% \end{proof}



==> other/offline.tex <==
\newcommand{\apr}{\mathsf{APR}}
\section{Offline}
First we consider the offline problem where all parameters of
the tasks are known ahead of time.
Schedulers for solving the offline problem besides being of
independent interest can also be used as subroutines in online
schedulers. We pick an optimal offline strategy and refer to
it as $\opt$.

Computing an exact solution can be done trivially via brute force
simulating every possible assignment of tasks to parallel or
serial. Note that deciding whether to run a task in serial or
parallel is all that must be done: without loss of generality
$\opt$ runs the serial jobs via \defn{most-work-first}, i.e. runs
up to $p$ of the serial jobs with the most remaining work at each
time slice, and runs the parallel jobs on any remaining
processors. 

First we give a scheduler for an important special case
\defn{single-arrival-time} TAPs, i.e. TAPs where 
all tasks arrive at the beginning.
\begin{proposition}
  \label{prop:singletime}
  There exists an optimal scheduler for single-arrival-time TAPs
  $\mathcal{T}$ with running time $O(n\lg n)$.
\end{proposition}
\begin{proof}
  We begin by sorting the tasks based on their serial works.
  Then, we compute in linear time serial work prefix sums
  $\sum_{i\leq k} \sigma_i$ and parallel work suffix sums
  $\sum_{i> k} \pi_i$ for all $k \in [n]$.
  Finally we compute in $O(n)$ time $$\min_{k\in [n]}
  \max\left(\sum_{i\leq k} \sigma_i/p + \sum_{i>k}\pi_i / p, \sigma_k\right),$$
  which is the minimum achievable awake time on this input TAP (achievable at the value of $k$ yielding the optimum). 
\end{proof}

Finding an exact solution to the full offline scheduling problem seems computationally intractable, so we focus on approximating it; in particular we give a polynomial approximation scheme.
\begin{proposition}
  For any $\eps > 0$, there exists an offline $1+\eps$ competitive scheduler with running time $\poly((pn/\eps^2)^{1/\eps})$ on TAP $\mathcal{T}$.
\end{proposition}
\begin{proof}
  We call our approximation algorithm $\apr$. We loop over each contiguous subset of the tasks $\mathcal{T}_{i}^{j}$ and determine the earliest time that these tasks can be completed (potentially with a $1+\eps$ factor error). $\opt$ will have gaps (times with no tasks) in between some contiguous subsets of tasks. Let $[a_1,b_1], [a_2,b_2],\ldots$ be such that $\opt$ has a gap between $b_i, a_{i+1}$ but no gap between any tasks in $[a_i,b_i]$. Let $\C_{\opt}^{\mathcal{T}_a^b}$ denote the time to complete tasks $\mathcal{T}_a^b$ (where we start counting time from $t_a$). Then we have:
  $$\T_{\opt}^{\mathcal{T}_1^n} = \sum_i
  \C_{\opt}^{\mathcal{T}_{a_i}^{b_i}}.$$
  Using our $1+\eps$ approximations to $\C_{\opt}^{\mathcal{T}_a^b}$ which we denote by $\C_{\apr}^{\mathcal{T}_a^b}$ we can achieve a schedule with awake time at most
  $$\sum_i (1+\eps)\C_{\opt}^{\mathcal{T}_{a_i}^{b_i}} \leq
  (1+\eps)\T_{\opt}^{\mathcal{T}_1^n}.$$
  In particular, once we have computed all values $\C_{\apr}^{\mathcal{T}_a^b}$ we use dynamic programming to compute a partition $[a_1',b_1'],[a_2',b_2'],\ldots$  of the tasks that optimizes 
  $$\sum_i \C_{\apr}^{\mathcal{T}_{a_i'}^{b_i'}}.$$
  Because $a_i'=a_i,b_i'=b_i$ is one such choice of partition this will certainly give us a $1+\eps$ approximation. It remains to describe how to compute 
  $$\C_{\apr}^{\mathcal{T}_{a}^{b}} \leq
  (1+\eps)\C_{\opt}^{\mathcal{T}_{a}^{b}}.$$
  For notational convenience in the following description we use $n$ instead of $b-a$ to denote the number of tasks in our subset of tasks.

  We reduce the optimization problem into a decision problem: repeatedly deciding whether or not the tasks can all be completed in time $\C$. This is possible because we can give a multiplicative range of size $p$ on the value of $\C$: let $\C_{\max}$ be the completion time if all tasks were run via parallel implementations, and $\C_{\opt}$ be the optimal completion time. Then
  $$\C_{\max}/p \leq \C_{\opt} \leq \C_{\max}.$$
  Now we demonstrate a procedure that if ${\C>(1+\eps)\C_{\opt}}$ states that finishing in time $\C$ is possible, and if $\C<\C_{\opt}$ outputs that finishing in time $\C$ is impossible. Using this procedure we can binary search to find a power of $(1+\eps)$ such that $(1+\eps)^i \leq \C_{\opt} \leq (1+\eps)^{i+1}.$ In particular, we must try $\log_{1+\eps}(p)\leq \O(\eps\lg p)$ values of $\C$ to get this $1+\eps$ approximation.

  Fix $\C$. Define the \defn{boundary times} to be $\C\eps \cdot i$ for $i\in 0,1,\ldots, 1/\eps$. We round the arrival times of tasks up to the nearest boundary time. We round the serial times which are at least $\eps \C/n$ large up to the nearest multiple of $\C\eps^2/n.$ We deal with all of the serial times less than $\eps \C / n$ in serial at the end, and so treat our new TAP as not having any of these incredibly small tasks. We claim that this rounding does not increase the optimum completion time by more than a factor of $(1+3\eps)$. Delaying all the tasks by $\C\eps$, multiplying all task sizes by $1+\eps$ and then adding $n \C\eps /n$ work at the end would increase the time by at most a factor of $1+3\eps$. This is an upper bound on how much we have increased the optimum work. By using $\eps' = \eps/3$ instead, we can ensure that the resulting TAP has optimum completion time at most a $1+\eps$ factor larger than before the rounding.

  Now we show how to exactly compute the optimum completion time of the rounded TAP via dynamic programming; this will complete the proof. We can represent a schedule of a prefix of the jobs by listing the amount of serial work present at each boundary time and listing the amount of parallel work present at the first boundary. Because of how the tasks sizes are rounded we require $p\cdot n/\eps^2$ possible values of serial work at each boundary. Thus, our DP table has size $(p\cdot n/\eps^2)^{1/\eps}.$  In each cell of the DP table we store whether or not this cell is possible, and if so, what the minimum parallel work is at the boundary time corresponding to the column in the DP for this serial arrangement. To fill the DP table we loop over the boundaries, and note the consequences of putting each task in serial or parallel via the DP.

  Overall the run time is $\poly((p\cdot n/\eps^2)^{1/\eps}).$
\end{proof}


==> other/parallel-work-obliv.tex <==
\section{A $4$-competitive Parallel Work Oblivious Scheduler}
Remarkably, we do not need to know the values $\pi_i$ to create a competitive schedule.
\begin{theorem}\label{thm:oblivpll2}
  There is a scheduler that is $2$ competitive
  for single arrival time TAPs without knowledge of parallel works.
\end{theorem}
\begin{proof}
  We call our algorithm $\til$. $\til$ starts by sorting the tasks so that $\sigma_1\geq \sigma_2\geq \cdots \geq \sigma_n$. $\til$ runs the largest task parallel until
  \begin{equation}
      \label{eq:tilswitch}
  \frac{t+\sigma_{i_*+1}}{t+\sum_{i>i_*}\sigma_i/p} = 2,
  \end{equation}
  and then schedules the remainder of the tasks in serial (these tasks are managed via most-work-first). Let $t_0$ be the time that $\til$ starts running serial tasks, and let $t' = \sum_{i\leq i_*}\pi_i/p$.
  $\opt$ must satisfy one of the following conditions: 
  
  \case{$\opt$ schedules one of the $i_*$ largest tasks in serial:}
  \begin{equation}
      \label{case2oblivA}
  \T_{\opt}\geq \sigma_{i_*}.
  \end{equation}
  \case{$\opt$ schedules all of the $i_*$ largest tasks in parallel:}
  \begin{equation}
  \label{case2oblivB}
  \T_{\opt}\geq t'+ \sum_{i>i_*}\sigma_i/p.
  \end{equation}
  We also note that $$\sigma_{i_*+1} = t_0 + 2\sum_{i>i_*}\sigma_i/p,$$
  due to \eqref{eq:tilswitch} and trivially $\T_{\opt} \geq \sum_i  \sigma_i /p.$

  Now we analyze the performance of $\til$ by considering four
  cases.
  
  \case{$\til$ ends jagged.} Then $\T_{\til} \leq t+\sigma_{i_*+1}$.\\
  In \cref{case2oblivA} we have:
  $$\T_{\til}\leq t+\sigma_{i_*+1} \leq 2\sigma_{i_*} \leq 2\T_{\opt},$$
  while in \cref{case2oblivB} we have:
  $$\T_{\til}\leq t+\sigma_{i_*+1} \leq 2\left(t+\sum_{i>i_*}\sigma_i/p\right)
  \leq 2\T_{\opt}.$$

  \case{$\til$ ends balanced.} Then $$\T_{\til}\leq
  t'+\sum_{i>i_*}\sigma_i/p.$$
  For \cref{case2oblivA} we have:
  $$\T_{\til}\leq t_0 + \pi_{i_*}/p + \sum_{i>i_*}\sigma_i/p \leq
  \T_{\opt} + \sigma_{i_*}\leq 2\T_{\opt},$$
  while for \cref{case2oblivB} we have:
  $$\T_{\til}\leq t'+\sum_{i>i_*}\sigma_i/p\leq \T_{\opt}.$$
\end{proof}

\noindent There is a simple generic method for turning single arrival time schedules into full schedules via batching.
\begin{lemma}
  \label{lem:batch}
  There is a transformation that turns a scheduler $\oracle_R$ which is
  $R$ competitive on single-arrival-time TAPs, into $\bat_R$ which
  is $2R$ competitive on general TAPs.
\end{lemma}
\begin{proof}
  $\bat_R$ operates as follows: whenever there are alive tasks
  but no currently running tasks, schedule a batch consisting of
  all alive tasks according to $\oracle_R$.
  Consider a TAP which causes $\bat_R$ to schedule batches at
  times $t_0,t_1, \ldots, t_n, t_{n+1}$. Without loss of
  generality we consider a TAP such that there are unfinished
  tasks at all times in $[t_0, t_{n+1}]$; any TAP can be split up
  into disjoint intervals where $\bat_R$ has alive tasks, and if $\bat_R$
  is competitive on one of these intervals it is certainly
  competitive on their union.
  The awake times for $\opt$ (times when $\opt$ has alive tasks)
  will be a collection of sub-intervals of this time range. Let
  $\T_{\opt}(t_{i},t_{i+1})$ denote the awake time of $\opt$ on the
  interval $[t_i, t_{i+1}]$. 

  We see that for $i\geq 1, t_{i+1}-t_i \leq R\cdot \T_{\opt}(t_{i-1},t_i)$.
  Intuitively, by waiting until a substantial amount of work
  arrives and then scheduling it all at once we avoid the
  possibility of making a decision that is bad because of a task
  that arrives when executing our decision. Also, $t_1-t_0 \leq R\cdot \T_{\opt}(t_0, t_1)$. 

  Adding this all together we achieve the desired result: 
  $$t_{n+1}-t_0 \leq 2R\cdot \T_{\opt}(t_0,t_n). $$
\end{proof}

Applying \cref{lem:batch} to \cref{thm:oblivpll2} gives:
\begin{corollary}
  There is a $4$-competitive PWO scheduler.
\end{corollary}

Another simple corollary of \cref{lem:batch} is:
\begin{corollary}
  There is a $2$-competitive vanilla scheduler.
\end{corollary}

